Acc-SpMM: Accelerating General-purpose Sparse Matrix-Matrix Multiplication with GPU Tensor Cores

General-purpose Sparse Matrix-Matrix Multiplication (SpMM) is a fundamental kernel in scientific computing and deep learning. The emergence of new matrix computation units such as Tensor Cores (TCs) brings more opportunities for SpMM acceleration. However, in order to fully unleash the power of hardware performance, systematic optimization is required. In this paper, we propose Acc-SpMM, a high-performance SpMM library on TCs, with multiple optimizations, including data-affinity-based reordering, memory efficient compressed format, high-throughput pipeline, and adaptive sparsity-aware load balancing. In contrast to the state-of-the-art SpMM kernels on various NVIDIA GPU architectures with a diverse range of benchmark matrices, Acc-SpMM achieves significant performance improvements, on average 2.52x (up to 5.11x) speedup on RTX 4090, on average 1.91x (up to 4.68x) speedup on A800, and on average 1.58x (up to 3.60x) speedup on H100 over cuSPARSE.

==> backup.tex <==


rom the table above, we can see that the instruction specification of m16n8k8 is more general. It can handle matrix calculations of FP16, TF32 and FP64 data types, so we chose the instruction of m16n8k8 specification for mma operation.
In tensor core mma computation, 
%1. 指令规格选取

% 通过上面的 table 可以知道，m16n8k8的指令规格更加通用，它可以处理 FP16、TF32 和 FP64的数据类型的矩阵计算，所以我们选用了 m16n8k8规格的指令进行mma运算。
%2. 转置
% （列出矩阵转置的式子），如果我们使用矩阵的转置计算，那么对于 ATile每次选取的规格就从 16 x 8 转换成了 8 x 8，如下表所示，可以进一步提升矩阵的稠密度，更好利用 tensor core 的特点对矩阵进行计算，更能整体上减少 mma 指令的调用次数。通过简单地交换线程行和列的取数规则可以直接对矩阵进行转置，只需要损失一部分几乎可以忽略不记的跨步取数的开销，但是却可以大大提高ATile 的稠密度。

The Table\ref{tab: improvement of density by transpose} shows mean NNZ in TC blocks and the improvement of density by transpose. It should be noted that the density is not obtained by directly dividing the average non-zero number, but by dividing the non-zero number by the TC block size. 

\noindent\textbf{Matrix transposition} Matrix multiplication $A \times B = C$ can be transformed with $(A \times B)^T = C^T$ which equals to $B^T \times A^T = C^T$, so we can simply compute matrix $C$ by $(B^T \times A^T)^T$. In tensor core mma computation, it only requires a simple swap of rows and columns to obtain the transposed matrix, we can simply change the position of each thread fetch data to achieve transposition of a matrix with minimal overhead. 


%3. 对于 cache 缓存策略的选择：如下表所示
% 由于矩阵B需要分成不同的片多次读入寄存器中，所以选择 .ca 对B进行缓存，可以更好利用 L1、L2 cache，加速矩阵取数的效率。对于矩阵A，由于异步拷贝的限制，我们选取了.ca对矩阵A进行读取。由于矩阵C在写回之后不再被用到，所以采用.wt指令的 写穿透机制对矩阵C进行写回，可以减少cache pollution，提高cache 的利用率和命中率。
\noindent\textbf{Cache policy control} As is shown in table.\ref{cache-control}, we can use PTX level instruction to control cache policy and increase the cache hit rate of the kernel. Due to the limit of async copy instruction, we can only choose to cache sparse matrix A both in L1 and L2 cache. For dense matrix B, we need to use it more than one time, so we cache it in L1 and L2 cache to minimize the load time of dense matrix B. 



To better use the cache of GPU, we choose .ca operator to load dense matrix B, and use .wt to write through dense matrix C in out kernel which will obtain a higher cache hit rate and avoid cache pollution with don't fetch again result C.

We use \textbf{mma.m16n8k8} to do our mma computation, and we mainly focus on tf32 datatype.


% 4. 流水：我们设计了一种流水方式可以尽可能多地进行数据掩盖，在预处理阶段，先load第一个 A tile，对应的 sparseAToB tile 0，和当前sparseAToB tile 对应的 dense B 矩阵。在正式的流水阶段，，使用异步操作取sparseA tile 和 sparseAToB tile，由于从 global memory 加载数据时间很长，所以可以用取dense B来overlap取sparseA ，取 sparseAToB 和计算。该流水方式可以做到充分掩盖取数和计算操作，效率最高。


% 解释下面的图：对于（a） 中的图首先进行dendrogram的构建，如（b）所示，先对图中的各个节点的度进行排序，从度最小的节点开始，寻找与其相邻节点是 deltaQ最小的节点进行合并，比如5，0节点进行合并，生成0’节点，更新0‘节点的度为4，再依次进行该系列操作，直到deltaQ <= 0 为止停止合并，（a）最终生成两颗独立的树，意味着原图被划分为两个社区。在此基础上，对dedrogram进行展开，按照 DFS的顺序遍历叶子节点，遍历到的叶子节点都在该社区内寻找与其具有公共邻居最多的相邻节点进行展开，比如节点5和节点7有一个公共邻居节点，数量最多，所以将节点7排在节点5的后面，标记节点7为visited，然后以节点7作为当前节点继续寻找与其公共邻居最多的相邻节点进行展开。对展开之后得到的序列进行节点的重新编号，从0开始，每次递增1，则成为新的节点编号。用新的节点编号之后的节点顺序对图进行重新排序，得到一个新的图，其对应的邻接矩阵如（e）所示，可以看到非零元的排布更加紧密了。

 Although our proposed Acc-SpMM is designed for tensor cores of NVIDIA GPUs with TP32 precision, our optimizations are able to be extended to other precisions and other acceleration devices with matrix computation units.
 For Type-1 matrices, matrix transposition multiplication is the crucial technique to achieve high performance.
